Beyond Words: On Large Language Models Actionability in Mission-Critical Risk Analysis

Context. Risk analysis assesses potential risks in specific scenarios. Risk analysis principles are context-less; the same methodology can be applied to a risk connected to health and information technology security. Risk analysis requires a vast knowledge of national and international regulations and standards and is time and effort-intensive. A large language model can quickly summarize information in less time than a human and can be fine-tuned to specific tasks. Aim. Our empirical study aims to investigate the effectiveness of Retrieval-Augmented Generation and fine-tuned LLM in risk analysis. To our knowledge, no prior study has explored its capabilities in risk analysis. Method. We manually curated 193 unique scenarios leading to 1283 representative samples from over 50 mission-critical analyses archived by the industrial context team in the last five years. We compared the base GPT-3.5 and GPT-4 models versus their Retrieval-Augmented Generation and fine-tuned counterparts. We employ two human experts as competitors of the models and three other human experts to review the models and the former human experts' analysis. The reviewers analyzed 5,000 scenario analyses. Results and Conclusions. Human experts demonstrated higher accuracy, but LLMs are quicker and more actionable. Moreover, our findings show that RAG-assisted LLMs have the lowest hallucination rates, effectively uncovering hidden risks and complementing human expertise. Thus, the choice of model depends on specific needs, with FTMs for accuracy, RAG for hidden risks discovery, and base models for comprehensiveness and actionability. Therefore, experts can leverage LLMs as an effective complementing companion in risk analysis within a condensed timeframe. They can also save costs by averting unnecessary expenses associated with implementing unwarranted countermeasures.

==> AnonymousAuthors.tex <==
\author{
\IEEEauthorblockN{Anonymous Authors}
\IEEEauthorblockA{
\textit{Affiliations}
}
}


==> Tables/WT/H04.tex <==


\begin{table}[tb]
\centering
\small
\caption{P-value and gain of the scenario metrics differences, i.e. H$_{04}$ test results.}
\label{tab:H04}
\begin{tabular}{lll}
\hline 
Metrics	& P-Value	& Gain\\
\hline
Actionable	& 0,0031	& 65\% \\
Comprehensive	& 0,2312	& 12\% \\
Extended GT &	0,0115	 & 28\% \\
\hline \\
\end{tabular}
\end{table}

==> Tables/confusion_matrix_definitions.tex <==
\begin{table}
    \centering
    \caption{Prediction Types}
    \begin{tabular}{@{}p{2.3cm}p{6.1cm}@{}}
    \hline
    Prediction Type & Description \\ \hline
    True Positive (TP) / False Positives (FP)& A vulnerability/threat is correctly identified in a scenario with that specific vulnerability/threat.    \\
    True Negative (TN) / False Negative (FN) & No vulnerability/threat is identified in a scenario that has no vulnerability/threat associated with it.     \\ \hline
    % False Positive (FP) &  A vulnerability/threat is incorrectly identified in a scenario without associated risks.  \\
    % False Negative (FN) & No vulnerability/threat is identified in a scenario with associated risks. \\ \hline
    \end{tabular}
    \label{tab:prediction_types}
\end{table}

==> Tables/mcc.tex <==
\begin{table}
    \centering
    \small
    \caption{Interpretation of MCC values.}
    \label{tab:mcc}
    \begin{tabular}{@{}ll@{}}
        \hline
        Value of MCC ($m$) & Interpretation \\
        \hline
         $0 \leq m < 0.2$ & Low \\
        $0.2 \leq m < 0.4$ & Fair \\
        $0.4 \leq m < 0.6$ & Moderate \\
        $0.6 \leq m < 0.8$ & Strong \\
        $0.8 \leq m < 1$ & Very Strong \\
        \hline
    \end{tabular}
\end{table}

==> Tables/metrics.tex <==
\begin{table}
  \centering
  \caption{IR Metrics}
  \label{tab:metrics}
  \begin{tabular}{lc|lc}
    \hline
\textbf{Metric} & \textbf{Formula}                                             & \textbf{Metric} & \textbf{Formula}      \\ \hline & & &\\
Accuracy        & $\dfrac{TP + FN}{TP+FP+TN+FN}$                               & Precision       & $\dfrac{TP}{TP + FP}$ \\& & &\\
F1-score        & $\dfrac{2 \cdot Precision \cdot Recall}{Precision + Recall}$ & Recall          & $\dfrac{TP}{TP + FN}$ \\ & & &\\ \hline
  \end{tabular}
\end{table}

%True positives + True Negatives)/ (True positives + True negatives + False positives + False negatives)
